Convergence of uncertainty estimates in Ensemble and Bayesian sparse model discovery

Sparse model identification enables nonlinear dynamical system discovery from data. However, the control of false discoveries for sparse model identification is challenging, especially in the low-data and high-noise limit. In this paper, we perform a theoretical study on ensemble sparse model discovery, which shows empirical success in terms of accuracy and robustness to noise. In particular, we analyse the bootstrapping-based sequential thresholding least-squares estimator. We show that this bootstrapping-based ensembling technique can perform a provably correct variable selection procedure with an exponential convergence rate of the error rate. In addition, we show that the ensemble sparse model discovery method can perform computationally efficient uncertainty estimation, compared to expensive Bayesian uncertainty quantification methods via MCMC. We demonstrate the convergence properties and connection to uncertainty quantification in various numerical studies on synthetic sparse linear regression and sparse model discovery. The experiments on sparse linear regression support that the bootstrapping-based sequential thresholding least-squares method has better performance for sparse variable selection compared to LASSO, thresholding least-squares, and bootstrapping-based LASSO. In the sparse model discovery experiment, we show that the bootstrapping-based sequential thresholding least-squares method can provide valid uncertainty quantification, converging to a delta measure centered around the true value with increased sample sizes. Finally, we highlight the improved robustness to hyperparameter selection under shifting noise and sparsity levels of the bootstrapping-based sequential thresholding least-squares method compared to other sparse regression methods.

==> bayesian_bootstrap.tex <==
The following content highlights some parts in paper \cite{clyde2001bagging}. 

\subsection{Bootstrap and Bagging}

Suppose we observe $n$ samples $X_1, ..., X_n$ for some distribution $F\in\mathcal{F}$. The parameter of interest is a functional $T(F)$. This functional $T(F)$ could be the mean, variance, median, and so on. For example, the mean could be defined as $\mu(F)=\int xdF$.

In frequentist's bootstrap \cite{efron1994introduction}, we estimate the entire functional using discrete samples $X_1, ..., X_n$, and set
\begin{align}
    F_n = \sum_{i=1}^n \omega_i \delta_{X_i}.
\end{align}


We access the distribution of $T(F)$ by repeatedly generating bootstrap replicates with $n$  with replacement sample drawn. 

The r-th bootstrap replicate $T(F^{(r)}_n)$ has $\omega^{(r)}_i \in \{0, \frac{1}{n}, \frac{2}{n}, \frac{n}{n}\}$. We sample $\omega$ using Multinomial distribution with $n$ bootstrap replicates and equal probability that $\omega\sim Multinom(n, p_1=\dots =p_n=\frac{1}{n})$. 

Bagging is coming from the $R$ bootstrap replicates. We have the bootstrap mean as
\begin{align*}
\bar{T}_R(F_n) &= \frac{1}{R} \sum_{r=1}^R T(F_n^{(r)}) \\ 
    &= \frac{1}{R} \sum_{r=1}^R \frac{\sum_{i=1}^n \omega_i^{(r)} X_i}{R}.
\end{align*}

\begin{lemma}
Bootstrap converges weakly to a deterministic limit
\end{lemma}


\subsection{Bayesian Bootstrap}

Bayesian bootstrap \cite{rubin1981bayesian} is nearly identical to frequentist bootstrap. We similarly estimate the entire functional using discrete samples $X_1, ..., X_n$ with weights $\omega$ and set

\begin{align}
    F_n = \sum_{i=1}^n \omega_i \delta_{X_i},\;\;\;\;\sum_i \omega_i = 1.
\end{align}

The only difference is coming from $\omega$. For bayesian bootstrap, $\omega_i\sim Dirichlet(1, 1, ..., 1)$. We may simply understand the Dirichlet distribution as a continuous version of Multinomial. We could see their relationship from Sec. \ref{sec:multi-dirichelet}. 

Notice $\omega_i$ in frequentist bootstrap can only be $\{0, \frac{1}{n}, \frac{2}{n}, ..., \frac{n}{n}\}$, but for $\omega_i$ in Bayesian bootstrap, $\omega_i \in [0, 1]$. 

We estimate the posterior distribution of $T(F)$ using Monte Carlo samples. First, we generate $\omega^{(b)} \sim Dirichlet(1, 1, ..., 1)$. Then, we calculate $T(F_n^{(b)})$ and obtain the posterior distribution of $T(F)$. 

Bagging will be considered as the posterior mean, and one could use Monte Carlo samples to estimate
\begin{align*}
\bar{T}_B(F_n) &= \frac{1}{B} \sum_{b=1}^B T(F_n^{(b)}) \\ 
    &= \frac{1}{B} \sum_{b=1}^B \frac{\sum_{i=1}^n \omega_i^{(b)} X_i}{B},
\end{align*}
where we have $B$ Monte Carlo samples of $\omega$ (and equivalently $T(F_n)$). 

Sometimes, people claim Efron's (frequentist) bootstrap is an \textbf{approximation} of Bayesian bootstrap. It is understandable that when we have infinite amount of $X_1, ..., X_n$ samples ($n\to\infty$), frequentist bootstrap is equivalent to Bayesian bootstrap. 

\subsubsection{Why can we sample from Dirichlet instead of Multinomial in Bayesian setting?} \label{sec:multi-dirichelet}

This subsection aims to relate Multinomial with Dirichlet. The following is just trying to plug-in prior and likelihood to Bayes formula. 

Bayesian bootstrap utilizes a prior 

\[
P(\omega) \propto \prod_{i=1}^n \omega_i^{-1}.
\]

We could see this prior as $Dirichlet(0, 0, ..., 0)$. 

From the samples $X_1, ..., X_n$, we know every $X_i$ is sampled once. Using a Multinomial likelihood with probability $\omega_i$ for each 
\[
N|\omega \sim Multinom(n, \omega).
\]

We have
\[
P(N|\omega) = \frac{n!}{N_1!...N_n!}\omega_1^{N_1}\omega_2^{N_2}\dots\omega_n^{N_n}.
\]

We can compute using Bayes formula that
\begin{align*}
P(\omega|N) &\propto P(\omega)P(N|\omega) \\
&= \frac{n!}{N_1!...N_n!}\omega_1^{N_1-1}\omega_2^{N_2-1}\dots\omega_n^{N_n-1}.
\end{align*}

We observe all $N_1=N_2=...=N_n$ (since these are our samples $X_1, ..., X_n$). We know the posterior is
\begin{align*}
P(\omega|N) &\propto\frac{n!}{N_1!...N_n!}\omega_1^{1-1}\omega_2^{1-1}\dots\omega_n^{1-1} \\
&= Const.
\end{align*}

Based on the constraint that $\sum\omega_i = 1$, we say that 
\[
\omega|N \sim Dirichlet(1,1,1, ..., 1).
\]

% \underline{Need to think more how to adapt this to E-SINDy setting.}

\section{Bootstrap LASSO}
Given samples $\{X_1, ..., X_n\}$. A key point here is that, the Bootstrap LASSO is \textbf{wrong} if the threshold $a_0$ is independent of $n$. Instead, we should construct $a_n=n^{-0.5}=\frac{1}{\sqrt{n}}$ (which satisfies certain condition like decreasing with more Bootstrap replicates) for thresholding. This allows convergence to the correct measure. 

In our case of E-SINDy, given a fixed number of samples $n$, picking a consistent $a_n$ for thresholding follows what this paper is saying, which is the correct thing. 

People call thresholding with this changing $a_n=\frac{1}{\sqrt{n}}$ modified Bootstrap LASSO. 

\begin{lemma}
Basic Bootstrap LASSO converges weakly to a random probability measure, unbiased mean but variance determined by a random process. 
\end{lemma}

\begin{lemma}
Modified Bootstrap LASSO converges weakly to the correct probability measure, unbiased mean and correct variance. 
\end{lemma}



==> bootstrapvs.tex <==
\begin{enumerate}
    \item Bootstrap Model Selection. Jun Shao, JASA, 1996.
    \item An asymptotic theory for linear model selection. Jun Shao, Statistica sinica, 1997.
    \item Spike and Slab Variable Selection: Frequentist and Bayesian Strategies. Hemant Ishwaran and J. Sunil Rao, AoS, 2005.
    \item Bootstrap LASSO Estimators. A. Chatterjee and S. N. Lahiri, JASA, 2011. 
    \item Thresholding least-squares inference in high-dimensional regression models. Mihai Giurcanu, EJS, 2016. 
\end{enumerate}

==> esindy.tex <==
\section{Ensemble SINDy variable selection framework}
\begin{enumerate}
    \item Construct Bootstrap replicates. 
    \item Estimate $\Xi^{(i)}$ with L2 regression and soft-thresholding. 
    \item Consider inclusion probability. 
\end{enumerate}

This question may split into two parts. 

(1) Bootstrap LASSO converges to the correct measure. Can we show L2 thresholding Bootstrap convergence to some correct thing (under some regularity condition)? 

1.1 Can Bootstrapping help with improving the FDR? Very likely. 

(2) We can perform inference to the inclusion probability, given some data generation model. Can we show this is the MLE? 

2.1 From paper "frequentist spike and slab", we know (yet need to prove by ourselves) OLS-HARD MODEL ESTIMATOR is asymptotic equivalent to THE ZCUT MODEL ESTIMATOR. 

2.2 The following step is just MLE. 

\subsection{Inclusion probability: some consideration}

Q: Is it possible to cast this process as an inference of $\ve{p}$? 

\begin{align*}
    \ve{y} &= \ve{X}\beta + \epsilon, \;\;\;\;\epsilon\sim\mathcal{N}(0, diag(\sigma_0)) \\
    \beta|\gamma &\sim \mathcal{N}(\mu(\gamma), \Sigma(\gamma)), \\
    \gamma &\sim Ber(\ve{p}).
\end{align*}

Denote $\circ$ as the Hadamard product, 
\[
\mu(\gamma) = \mu\circ\gamma, \Sigma(\gamma) = diag(\sigma\circ\gamma). 
\]

The MLE of $\ve{p}$, given $\ve{\gamma_1}, ..., \ve{\gamma_n}$, is simply
\[
\ve{p} = \frac{\sum \ve{\gamma_i}}{n}.
\]

How can we inference $\gamma$? 

Let's think of the following inference structure by identifying the non-active terms. 

\section{Thresholding least-squares~\cite{giurcanu2016thresholding}}

The setting is from Mihai Giurcanu who build up everything together. The following contents are highlights from his paper. 

Consider linear regression: 

\[
Y_{i}=X_{i}^{T}\beta+\epsilon_{i},\;\;\;\;i=1,...,n.
\]

Consider the standardized and certered version, we see $\bar{Y}=0,\bar{X}^{(j)}=0,$
and $\bar{S}^{(j)}=1$, where

\[
\bar{Y}=n^{-1}\sum_{i}Y_{i},\;\;\;\;\bar{X}^{(j)}=n^{-1}\sum_{i}X_{ij},\;\;\;\;\bar{S}^{(j)}=n^{-1}\sum_{i}X_{ij}^{2},\;\;\;\;j=1,...,p.
\]

Let $I=\text{\{}1,...,p\text{\}}$. 

Let $b=(b_{1},...,b_{p})^{T}\in\mathbb{R}^{p}.$

Let $K_{b}=\text{\{\ensuremath{j\in I:b_{j}=0}\}}$, $J_{b}=\text{\{\ensuremath{j\in I:b_{j}\neq0}\}}$. 

Let $q_{J}=card(J)$. 

Let $\Theta_{1}$ be all the sprase solutions, $\mathbb{R}^{p}\backslash\Theta_{1}$
be all the non-sparse solutions. 

\subsection{Case $p<n$}

First consider OLS that

\[
\bar{\beta}=(X^{T}X)^{-1}X^{T}Y=n^{-1}\Omega^{-1}\sum_{i}X_{i}Y_{i}=\sum_{i}c_{i}Y_{i},
\]

where $X=(X_{ij})\in\mathbb{R}^{n\times p}$ is the design, $c_{i}=(X^{T}X)^{-1}X_{i}\in\mathbb{R}^{p\times p}$,
and

\[
\Omega=n^{-1}X^{T}X=n^{-1}\sum_{i}X_{i}X_{i}^{T}\in\mathbb{R}^{p\times p}.
\]

And unbiased OLS of $\sigma^{2}$ is

\[
\bar{\sigma}^{2}=\frac{1}{n-p}\sum_{i}(Y_{i}-X_{i}^{T}\bar{\beta})^{2}.
\]

Let $\rho_{1},\rho_{2}$ denote the min and max eigenvalues of $\Omega$,
and let $||a||$ denote the Euclidean norm of $a\in\mathbb{R}^{p}$.
We assume the following regularity conditions: 

A.1 $\mathbb{E}(\epsilon)=0$, $var(\epsilon)=\sigma^{2}$, and $\mathbb{E}(\epsilon^{4})<\infty$,
where $\epsilon\sim P$. 

A.2 $\rho_{1}>0$, $\max_{i\leq i\leq n}||X_{i}||^{2}=O(p),$and $p/(n\rho_{1})=o(1)$. 

Note here since $tr(\Omega)=p$, then $\rho_{1}\leq1$. By A.2, we
know $p=o(n)$. The following Lemma depicts the consistency of $\bar{\beta},\bar{\sigma}^{2}$. 
\begin{lemma}
Suppose that conditions A.1 and A.2 hold and let $a\in\mathbb{R}^{p}$
with $||a||=1$. Then 

i. $a^{T}(\bar{\beta}-\beta)=O_{P}((\rho_{1}n)^{-1/2})$

ii. $\bar{\sigma}^{2}=\sigma^{2}+O_{P}(n^{-1/2})$
\end{lemma}

The following Lemma shows that $a^{T}\bar{\beta}$ is asymptotic normal
for all $a\in\mathbb{R}^{p}$ with $||a||=1$. 
\begin{lemma}
Suppose that conditions A.1 and A.2 and let $a\in\mathbb{R}^{p}$
with $||a||=1$. Then

\[
\bar{s}^{-1/2}a^{T}(\bar{\beta}-\beta)\xrightarrow{d}\mathcal{N}(0,1),
\]

where $\bar{s}=n^{-1}\bar{\sigma}^{2}a^{T}\Omega^{-1}a$. 
\end{lemma}

For $J\subseteq I$, let $\beta_{J}=(\beta_{j}:j\in J)^{T}\in\mathbb{R}^{q_{J}}$,
$X_{J}=(X_{ij}:1\leq i\leq n,j\in J)\in\mathbb{R}^{n\times q_{J}}$,
$\Omega_{JK}=n^{-1}X_{J}^{T}X_{K}\in\mathbb{R}^{q_{J}\times q_{K}}$,
and let

\[
\Sigma_{KK}=\Omega_{KK}-\Omega_{KJ}\Omega_{JJ}^{-1}\Omega_{JK}\in\mathbb{R}^{q_{K}\times q_{K}},
\]

where $K=I\backslash J$. 

An immediate consequence of Lemma 2 is that for every fixed $K\subset K_{\beta}$
(i.e., $K$ does not depend on $n$), we have

\[
n^{1/2}\bar{\sigma}^{-1}\Sigma_{KK}^{1/2}(\bar{\beta}_{K}-\beta_{K})\xrightarrow{d}\mathcal{N}(0,I_{qk}).
\]

Note that the F-test statistics for testing $H_{0}:K_{\beta}=K$ against
$H_{a}:K_{\beta}\neq K$, where $K\subset I$ is fixed, is given by

\[
\hat{F}(K)=n\frac{\bar{\beta}_{K}^{T}\Sigma_{KK}\bar{\beta}_{K}}{q_{K}\bar{\sigma}^{2}}.
\]

We could use a chi-squared distribution that

\[
q_{K}\hat{F}(K)\xrightarrow{d}\chi_{q_{K}}^{2}.
\]

\begin{lemma}
Suppose conditions A.1, A.2 hold and $n\rho_{1}^{2}\to\infty$. Then,
under $H_{0}:K_{\beta}=K$, 

\[
\frac{q_{K}\hat{F}(K)-q_{K}}{(2q_{K})^{1/2}}\xrightarrow{d}\mathcal{N}(0,1).
\]
\end{lemma}

Let $\hat{K}$ be a thresholding estimator of the index set of the
zero components of $\beta,K_{\beta}$, given by

\[
\hat{K}=\text{\{}j\in I:|\bar{\beta}_{j}|\leq\gamma\bar{\sigma}_{jj}\text{\}},
\]

where $\bar{\beta}=(\bar{\beta}_{j}:j\in I)^{T}\in\mathbb{R}^{p}$,
$\gamma$ is the thresholding parameter, $\bar{\sigma}_{jj}=n^{-1/2}\bar{\sigma}\omega_{jj}^{1/2},$
and $\Omega^{-1}=(\omega_{ij})\in\mathbb{R}^{p\times p}$. We assume
that $\gamma$satisfies the following conditions: 

(2.4a)
\[
\frac{\rho_{1}\rho_{2}^{-1}\gamma^{2}-q_{K_{\beta}}}{q_{K_{\beta}}^{1/2}}\to\infty
\]

and

(2.4b)

\[
\frac{\rho_{1}\rho_{2}^{-1}(n^{1/2}\sigma^{-1}\rho_{1}^{1/2}\min_{j\in J_{\beta}}|\beta_{j}|-\gamma)^{2}-q}{q^{1/2}}\to\infty.
\]

How to interpret these conditions? 

Suppose for the moment that $\lim\inf_{n}\rho_{1}>0$, $\lim\inf_{n}\rho_{2}^{-1}>0$,
$\lim\inf_{n}\min_{j\in J_{\beta}}|\beta_{j}|>0$, and $q_{K_{\beta}}\sim n^{\tau}$,
where $0<\tau<1$. We setup $\gamma=(p\log(p))^{1/2}$ and $p=o(n/\log(n))$. 

The TLSE of $\beta$ is defined as 

\[
\hat{\beta}=\arg\min_{b\in\mathbb{R}^{p}}\text{\{}(Y-Xb)^{T}(Y-Xb):b_{\hat{K}}=0\text{\}}.
\]

Note that $\hat{\beta}_{\hat{K}}=0$, $\hat{\beta}_{\hat{J}}=(X_{\hat{J}}^{T}X_{\hat{J}})^{-1}X_{\hat{J}}^{T}Y$,
where $\hat{J}=I\backslash\hat{K}$. Let further 

\[
\hat{\sigma}^{2}=\frac{1}{n-q_{j}}\sum_{i=1}^{n}(Y_{i}-X_{i}^{T}\hat{\beta})^{2}
\]

be the TLSE of $\sigma^{2}$. The following Theorem shows that TLSE
has similar asymptotic properties as the LASSO-type estimators that
have the oracle property. 
\begin{theorem}
Suppose that conditions A.1, A.2, (2.4a), (2.4b) hold, and that $n\rho_{1}^{2}\to\infty$.
Then $\hat{\beta}$ has the oracle property, i.e., 

(i) $Pr(\hat{K}=K_{\beta})\to1$; 

(ii) $\hat{s}^{-1/2}a^{T}(\hat{\beta}-\beta)\xrightarrow{d}\mathcal{N}(0,1)$,
where $a\in\mathbb{R}^{p},||a||=1$, and $\hat{s}=n^{-1}\hat{\sigma}^{2}a_{\hat{J}}^{T}\Omega_{\hat{J}\hat{J}}^{-1}a_{\hat{J}}.$ 
\end{theorem}

We further have the following Corollary. 
\begin{corollary}
Suppose conditions A.1, A.2, (2.4a), (2.4b) hold and that $n\rho_{1}^{2}\to\infty$.
Then $\hat{\beta}$ is asymptotically at least as efficient as $\hat{\beta}$.
\end{corollary}

We go through the proof of Theorem 4. 

\subsection{Bootstrap inference}

Let $\hat{\beta}$ be the bootstrap version of $\beta$ in the context
of thresholding least-squares inference. Let $\hat{\epsilon}_{i}=Y_{i}-X_{i}^{T}\hat{\beta}$
be the ith (raw) residual; since $\bar{X}=0$ and $\bar{Y}=0$, then
$\sum_{j=1}^{n}\hat{\epsilon}_{j}=0$, and thus, the residuals are
inherently ``centered'' at zero. Let $\hat{E}_{1:n}=\text{\{}\hat{\epsilon}_{1},...,\hat{\epsilon}_{n}\text{\}}$
be the sample of residuals and let $\mathbb{P}=n^{-1}\sum_{i=1}^{n}\delta_{\epsilon_{i}}$
denote the empirical distribution. The bootstrap version of $\hat{\beta}$
is 

\[
\hat{\beta}^{*}=\arg\min_{b\in\mathbb{R}^{p}}\left\{ (Y^{*}-Xb)^{T}(Y^{*}-Xb):b_{\hat{K}}=0\right\} .
\]

\begin{theorem}
Suppose that conditions A.1, A.2, (2.4a), (2.4b) hold, and that $n\rho_{1}^{2}\to\infty$.
Then

(i) $\mathscr{L}(\hat{s}^{*-1/2}a^{T}(\hat{\beta}^{*}-\hat{\beta})|Y)\xrightarrow{Pr}\mathcal{N}(0,1)$
for $\beta\in\Theta$. 

Suppose further that $\lim\sup_{n}\rho_{1}^{-1}\rho_{2}<\infty$.
Then, 

(ii) $\mathscr{L}(\hat{s}^{*-1/2}a^{T}(\hat{\beta}^{*}-\bar{\beta})|Y)\xrightarrow{d}\mathcal{N}(Z,1)$
for $\beta\in\Theta_{1}$, where $Z\sim\mathcal{N}(0,\sigma_{\eta}^{2})$. 
\end{theorem}

\subsection{Further guarantee focusing on Bootstrap}

\begin{question} [Method 1]
 An easy way is to consider the setting that
 \[
 \hat{K}^* = \left\{j\in I : \left| \frac{1}{n} \sum_{b=1}^n \beta_j^b \right| \leq \gamma n^{-1/2} \hat\sigma^* \omega_{jj}^{1/2} \right\}.
 \]
 Are we able to show that 
 \[
 Pr(\hat{K}^* = K_\beta) \to 1,
 \]
 with less amount of sample, i.e. to relax the large sample assumption that $\frac{p}{n\rho_1} = o(1)$? 
\end{question}

There may have minor hope for M1 setting since bootstrap for OLS would enlarge the variance. It is possible to shrink but the additional assumption will break Lemma 3 then Thm. 1 will be much harder to prove.

\vspace{5mm}

\begin{question} [Method 1.5: an variant]
 An easy way is to consider the setting that
 \[
 \hat{K}^* = \left\{j\in I : \left| \frac{1}{n} \sum_{b=1}^n \hat{\beta}_j^b \right| \leq \gamma n^{-1/2} \hat\sigma^* \omega_{jj}^{1/2} \right\},
 \]
 and 
 \[
 \hat{\beta}_j = \begin{cases}0, |\bar{\beta}_j| \leq \gamma\bar{\sigma}_{jj},\\
 \bar{\beta}_j, otherwise.
 \end{cases}
 \]
\end{question}

\vspace{5mm}

Start from the initial version of proof... 

\begin{proof}
Let $\Xi_{K_\beta K_\beta}=diag(\Sigma_{K_\beta K_\beta}^{-1})$ be the diagonal matrix of $\Sigma^{-1}_{K_\beta K_\beta}=(\Omega^{-1})_{K_\beta K_\beta}$. 

Since $\Sigma_{K_\beta K_\beta}^{-1}$ is the diagonal submatrix of $\Omega^{-1}$, we have the spectral norm $||\Sigma^{-1}_{K_\beta K_\beta}||_2 \leq ||\Omega^{-1}||_2 = \rho_1^{-1}$. Further because $\Xi_{K_\beta K_\beta}$ is diagonal submatrix of $\Sigma_{K_\beta K_\beta}^{-1}$, we have

\[
\lambda_{\min}(\Xi_{K_\beta K_\beta}) \geq \lambda_{\min}(\Sigma^{-1}_{K_\beta K_\beta}) \geq \lambda_{\min}(\Omega^{-1}) = \rho_2^{-1}.
\]

We further have
\[
||\Xi^{-1}_{K_\beta K_\beta}||_2 \leq \rho_2.
\]

\textbf{Step 1: Show $Pr(K_\beta \subset K) \to 1$.}

First, recall $K_\beta$ are all the non-active elements. 

\begin{align*}
    Pr\lrp{\max_{j\in K_\beta} \frac{|\bar{\beta}_j|}{\bar{\sigma}_{jj}} \geq \gamma} \leq Pr\lrp{\sum_{j\in K_\beta} \frac{\bar{\beta}^2_j}{\bar{\sigma}^2_{jj}} \geq \gamma^2}. 
\end{align*}

\begin{align*}
    Pr\lrp{\max_{j\in K_\beta} \frac{|\frac{1}{n}\sum_{b=1}^n \ind{\bar{\beta}^b_j \leq \gamma\bar{\sigma}^b_{jj}}\bar{\beta}^b_j|}{\bar{\sigma}_{jj}} \geq \gamma} &\leq 
\end{align*}

Consider about this quantity independently, 
\begin{align*}
    |\frac{1}{n}\sum_{b=1}^n \ind{\bar{\beta}^b_j \leq \gamma\bar{\sigma}^b_{jj}}\bar{\beta}^b_j|.
\end{align*}

It turns out that we could consider 
\[
\Ep{\bar{\beta}_j^b \sim Gaussian, \bar{\sigma}_j^b\sim Chi-square}{\bar{\beta}_j^b \ind{\bar{\beta}^b_j\leq \gamma \bar{\sigma}^b_j}}
\]

We first denote the LSE solution has the property that
\[
(\bar{\beta} - \beta) = O_P((\rho_1 n)^{-1/2}),\;\bar{\sigma}^2 = \sigma^2 + O_P(n^{-1/2}). 
\]

And, 
\[
n^{1/2}\bar{\sigma}^{-1}\Sigma_{KK}(\bar{\beta}_K-\beta_K) \xrightarrow[]{d} \mathcal{N}(0, I).
\]


\end{proof}

\begin{question} [Method 2]
 Another way is that, given bootstrapped $\hat{K}$ that $\{\hat{K}^1, ..., \hat{K}^b, ..., \hat{K}^n\}$, 
 \[
 \hat{K}^* = \left\{j\in I : \frac{\sum_{i=1}^n \ind{j\in \hat{K}^i}}{n} < \delta\right\}.
 \]
 Are we able to show 
 \[
 Pr(\hat{K}^* = K_\beta) \to 1,
 \]
 with less amount of sample, i.e. to relax the large sample assumption that $\frac{p}{n\rho_1} = o(1)$? 
\end{question}

There are some hope here from 'Analyzing bagging' by Peter Bühlmann, Bin Yu from AoS, 2002.

\vspace{5mm}


\begin{question}
 Can we show Question 1 and Question 2 are equivalent? 
\end{question}

\subsection{Gaussian noise assumption}
\input{gaussian_non_asymptotic.tex}

==> gaussian_non_asymptotic.tex <==
First consider OLS that

\[
\bar{\beta}=(X^{T}X)^{-1}X^{T}Y=n^{-1}\Omega^{-1}\sum_{i}X_{i}Y_{i}=\sum_{i}c_{i}Y_{i},
\]

where $X=(X_{ij})\in\mathbb{R}^{n\times p}$ is the design, $c_{i}=(X^{T}X)^{-1}X_{i}\in\mathbb{R}^{p\times p}$,
and

\[
\Omega=n^{-1}X^{T}X=n^{-1}\sum_{i}X_{i}X_{i}^{T}\in\mathbb{R}^{p\times p}.
\]

And unbiased OLS of $\sigma^{2}$ is

\[
\bar{\sigma}^{2}=\frac{1}{n-p}\sum_{i}(Y_{i}-X_{i}^{T}\bar{\beta})^{2}.
\]

Let $\rho_{1},\rho_{2}$ denote the min and max eigenvalues of $\Omega$,
and let $||a||$ denote the Euclidean norm of $a\in\mathbb{R}^{p}$.
We assume the following regularity conditions: 

A.1 $\epsilon\sim \mathcal{N}(0, \sigma^2 I)$. 

A.2 $\rho_{1}>0$, $\max_{i\leq i\leq n}||X_{i}||^{2}=O(p),$and $p/(n\rho_{1})=o(1)$. 

Note here since $tr(\Omega)=p$, then $\rho_{1}\leq1$. By A.2, we
know $p=o(n)$. The following Lemma depicts the consistency of $\bar{\beta},\bar{\sigma}^{2}$. 


The following Lemma shows that $a^{T}\bar{\beta}$ is asymptotic normal
for all $a\in\mathbb{R}^{p}$ with $||a||=1$. 
\begin{lemma}
Suppose that conditions A.1 and A.2 and let $a\in\mathbb{R}^{p}$
with $||a||=1$. Then

\[
n^{1/2}(\bar{\beta}-\beta)\xrightarrow{d}\mathcal{N}(0,\bar{\sigma}^{2}(X^TX)^{-1}),
\]
and we have
\[
\mathbb{P}\lrp{(\bar\beta-\beta) \geq \sqrt{\frac{2\bar{\sigma}^{2}(X^TX)^{-1}\log(1/\delta)}{n}}} \leq \delta.
\]
\end{lemma}

We further have with probability at least $1-\delta$, 
\[
(\bar\beta-\beta) \leq \bar{\sigma}\sqrt{\frac{2(X^TX)^{-1}\log(1/\delta)}{n}}. 
\]

For $J\subseteq I$, let $\beta_{J}=(\beta_{j}:j\in J)^{T}\in\mathbb{R}^{q_{J}}$,
$X_{J}=(X_{ij}:1\leq i\leq n,j\in J)\in\mathbb{R}^{n\times q_{J}}$,
$\Omega_{JK}=n^{-1}X_{J}^{T}X_{K}\in\mathbb{R}^{q_{J}\times q_{K}}$,
and let

\[
\Sigma_{KK}=\Omega_{KK}-\Omega_{KJ}\Omega_{JJ}^{-1}\Omega_{JK}\in\mathbb{R}^{q_{K}\times q_{K}},
\]

where $K=I\backslash J$. 

An immediate consequence of Lemma 4 is that for every fixed $K\subset K_{\beta}$
(i.e., $K$ does not depend on $n$), we have

\[
n^{1/2}\bar{\sigma}^{-1}\Sigma_{KK}^{1/2}(\bar{\beta}_{K}-\beta_{K})\xrightarrow{d}\mathcal{N}(0,I_{qk}).
\]

Using similar Gaussian tail bound, we know w.p. $1-\delta$, 

\[
(\bar{\beta}_{K}-\beta_K) \leq n^{-1/2}\bar{\sigma}\sqrt{\frac{2(X^TX)^{-1} \log(1/\delta)}{n}}
\]

From here, suppose we have 

\[
\hat{F}(K) = n\frac{\bar\beta_K^T \Sigma_{KK}\bar\beta_K}{q_K}.
\]

We see here that

\[
q_K\hat{F}(K) \xrightarrow[]{d} \chi^2_{q_K}.
\]



Similarly, we could set that 
\[
\hat{K} = \{j\in I: |\bar{\beta}_j| \leq n^{-1/2}\bar{\sigma}\sqrt{2(X_j^TX_j)^{-1}\log(1/\delta)}\}.
\]

If variance is assumed to be know and WLOG $\sigma^2=1$, we have $\hat{K}$ to be 
\[
\hat{K} = \{j\in I: |\bar{\beta}_j| \leq n^{-1/2}\sqrt{2(X_j^TX_j)^{-1}\log(1/\delta)}\}.
\]

\[
(\bar{\beta}_{j}-\beta_j) \sim \mathcal{N}\lrp{0, \frac{(X_j^TX_j)^{-1}}{n}}. 
\]

Consider here that 
\begin{align*}
    Pr\lrp{\max_{j\in K_\beta} |\bar{\beta}_j| > n^{-1/2}\sqrt{2(X^T_jX_j)^{-1}\log(1/\delta)}} &= Pr\lrp{\frac{1}{\sqrt{\log(1/\delta)}}n\bar{\beta}_{K_\beta}^T\Xi^{-1}_{K_\beta}\bar{\beta}_{K_\beta} \geq 1} \\
    &\leq Pr\lrp{\frac{1}{\sqrt{\log(1/\delta)}} q_{K_\beta}\rho_2\rho_1^{-1}\hat{F}(K_\beta) \geq 1} \\
    &= Pr\lrp{q_{K_\beta}\hat{F}(K_\beta) \geq \rho_1\rho_2^{-1}\sqrt{\log(1/ \delta)}}.
\end{align*}

What would be the difference if we do Bootstrap? There is a (cute) plotting in Fig. \ref{fig:term1_convergence_rate} considering the false discovery rate. Bootstrapping Thresholding OLS is much better that \textbf{with smaller sample size, it will not falsely treat a non-active term as something active}.  

This motivates the following analysis: 

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{figs/term1_convergence_rate.png}
    \caption{False discovery rates of Ordinary Least-Square (OLS), Bootstrapping OLS, and Bootstrapping thresholding OLS. }
    \label{fig:term1_convergence_rate}
\end{figure*}

\begin{align*}
    &Pr\lrp{\max_{j\in K_\beta} \left|\frac{1}{n}\sum_{b=1}^n \bar{\beta}^b_j\ind{\bar\beta^b_j \leq n^{-1/2}\sqrt{2(X^{bT}_jX^b_j)^{-1}\log(1/\delta)}}\right| > n^{-1/2}\sqrt{2(X^T_jX_j)^{-1}\log(1/\delta)}} \\
    &= Pr\lrp{\max_{j\in K_\beta} \left|\delta \E{\bar{\beta}^b_j 
    \ind{\bar{\beta}^b_j \geq n^{-1/2}\sqrt{2(X^{bT}_jX^b_j)^{-1}\log(1/\delta)}}}\right| > n^{-1/2}\sqrt{2(X^T_jX_j)^{-1}\log(1/\delta)}} \\
    &= Pr\lrp{\max_{j\in K_\beta} \left| \E{\bar{\beta}^b_j 
    \ind{\bar{\beta}^b_j \geq n^{-1/2}\sqrt{2(X^{bT}_jX^b_j)^{-1}\log(1/\delta)}}}\right| > \frac{n^{-1/2}}{\delta}\sqrt{2(X^T_jX_j)^{-1}\log(1/\delta)}}
\end{align*}

Consider this quantity, 
\begin{align*}
    \textbf{B}_j = \frac{1}{n} \sum_{b=1}^n \bar{\beta}^b_j 
    \ind{\bar{\beta}^b_j \geq \sqrt{2(X^{T}_jX_j)^{-1}\log(1/\delta)}}
\end{align*}

We can know $\Ep{\omega_i\sim Mul(n, \frac{1}{n})}{\textbf{B}_j} = 0$ by seeing $\bar{\beta}_j^b - \bar{\beta}_j\sim\mathcal{N}(0, \theta_0^2)$ and $\bar{\beta}_j - \beta_j\sim\mathcal{N}(0, \theta_0^2)$. Therefore, $\bar\beta^b_j-\beta_j\sim\mathcal{N}(0, 2\sigma^2)$. 

What would be the variance? The variance term by definition is
\begin{align*}
    Var[\mathbf{B}_j] &= \int_{x\in\mathbb{R}} x^2p(x)dx \\
    &= 2\int_{x>\sqrt{2\sigma^2\log(1/\delta)}}^{+\infty} x^2 p(x) dx \\
    &= 2\int_{x>\sqrt{2\sigma^2\log(1/\delta)}}^{+\infty} x^2 p(x) dx \\
    &= 2\sigma^2\lrp{erfc\lrp{\frac{1}{\sqrt{2\log(1/\delta)}}} + \sqrt{\frac{2}{e\pi}}} \\
    &= 2\sigma^2\lrp{erfc\lrp{\frac{1}{\sqrt{2\log(1/\delta)}}} + \sqrt{\frac{2}{e\pi}}} \\
    \sigma[\mathbf{B}_j]&= \sqrt{2(X_j^TX_j)^{-1}\lrp{erfc\lrp{\frac{1}{\sqrt{2\log(1/\delta)}}} + \sqrt{\frac{2}{e\pi}}}}
\end{align*}

Using Chebyshev we know that
\begin{align*}
    Pr\lrp{|\mathbf{B}_j| \geq \sqrt{2(X_j^TX_j)^{-1}\log(1/\delta)}} &= Pr\lrp{|\mathbf{B}_j| \geq \sigma[\mathbf{B}_j]\cdot \frac{\sqrt{\log(1/\delta)}}{\sqrt{erfc\lrp{\frac{1}{\sqrt{2\log(1/\delta)}}}+\frac{2}{e\pi}}}} \\
    &\leq \frac{erfc(\frac{1}{\sqrt{2\log(1/\delta)}})+\frac{2}{e\pi}}{\log(1/\delta)} \\
    &= 0
\end{align*}

The replication of this process for $q$ times, if we consider 
\begin{align*}
    Pr\lrp{\max_{j\in K_\beta} |\mathbf{B}_j| \geq \sqrt{2(X_j^TX_j)^{-1}\log(1/\delta)}} &= Pr\lrp{|\mathbf{B}_j| \geq \sigma[\mathbf{B}_j]\cdot \frac{\sqrt{\log(1/\delta)}}{\sqrt{erfc\lrp{\frac{1}{\sqrt{2\log(1/\delta)}}}+\frac{2}{e\pi}}}} \\
    &\leq \frac{erfc(\frac{1}{\sqrt{2\log(1/\delta)}})+\frac{2}{e\pi}}{\log(1/\delta)} \\
    &= 0
\end{align*}

\textbf{It is reasonable to assume that $q/n=o(1)$ and the problems can be solved.}

\subsection{Other side of the bound and (2.4b) assumption}

We don't necessary need to improve this part. But we can do this from M2 setting.

\begin{align*}
    Pr\lrp{\min_{j\in J_\beta} |\bar{\beta_j}| \leq \sqrt{2(X_j^TX_j)^{-1}\log(1/\delta)}}
\end{align*}

==> intro.tex <==
Governing equation discovery is essential for physical science. In the modern era of big data, an incredible amount of data gives rise to opportunities to perform data-driven model discovery~\citep{schmidt2009distilling} based on the first principle, which is widely applicable for scientific problems including neuroscience, epidemiology, astronomy, robotics, and so on. 
Even if there have been many discussions about model discovery algorithms, sparse regression methods are one of the most popular methods due to their simplicity in implementation, efficiency in computation, and robustness in accuracy.
The sparse identification of nonlinear dynamics algorithm (SINDy)~\citep{brunton2016discovering} utilizes sequential Thresholding Least-square Estimator (TLSE) to promote sparsity. 
More recently, Fasel et al.~\citep{fasel2022ensemble} propose Ensemble SINDy (E-SINDy) which constructs bootstrap replicates generated from the TLSE-based variable selection. With the Bootstrapping step, E-SINDy not only enables uncertainty quantification in parametric inference, but also empirically improves the robustness of variable selection under limited and noisy data. Even if E-SINDy algorithms achieve huge success from the engineering perspective, a theoretical understanding is missing to explain the improvements. 
In this paper, we study a theoretical extension of E-SINDy for sparse linear regression by analyzing a bagging inclusion probability based Thresholding Least-squares Estimation. We prove that the E-SINDy algorithm is able to perform correct sparse model identification through the exponential convergence of False discovery probability (FDP) and True discovery probability (TDP). The theoretical result on the correct sparse identification additionally offers a statistical guarantee on the uncertainty quantification of E-SINDy. These theoretical results reveal the effectiveness of E-SINDy for sparse model discovery, and the potential as a general sparse linear regression method. 

% \begin{figure*}
%     \includegraphics[width=0.95\textwidth]{paper/figs/informal_Thm_1.pdf}
%     \caption{We observe exponential convergence for Bagging inclusion probability TLSE of Empirical False Discovery Probability (EFDP) and Empirical True Discovery Probability (ETDP). The orange curve is a dominated by $\exp(-\alpha\cdot n)$ where $\alpha$ is a constant. } 
%     \label{fig:informal_thm1}
% \end{figure*}



From the standpoint of variable selection, it is nontrivial to derive the theoretical guarantee of SINDy and E-SINDy as thresholding procedures. Most literature alternatively focuses on the least absolute shrinkage and selection operator (LASSO)~\citep{tibshirani1996regression} which utilizes an $\ell_1$ shrinkage estimator for sparse regression. The statistical properties of LASSO-based methods have been systematically studied, including the consistency~\citep{zhao2006model}, the oracle property in classic regression settings~\citep{fan2001variable,zou2006adaptive}, and in high-dimensional settings~\citep{wainwright2019high,huang2008asymptotic}. 
From the Bayesian perspective, a hierarchical Bayesian model with Spike-and-slab~\citep{mitchell1988bayesian,george1997approaches,ishwaran2005spike} or regularized horseshoe prior~\citep{carvalho2009handling,carvalho2010horseshoe} are thoroughly studied with the effectiveness for Bayesian sparse inference. 
Even if thresholding-based methods achieve good performances in many problems~\citep{donoho1994ideal,donoho1995noising,bhatia2015robust}, the development of its statistical foundation is not fully established. 
Only until recently, Giurcanu propose a statistical understanding of thresholding-based estimators~\citep{giurcanu2016thresholding}, and show statistical guarantees of the thresholding-based estimatior in sparse variable selection.

% Exchange a <-> b
% TDP CAP not consistetn
\begin{figure*}[!ht]
    \includegraphics[width=\textwidth]{paper/figs/Fig1_revised.pdf}
    \caption{(a) Top: evolution of distributional estimation of the E-SINDy algorithm over different sample sizes. Bottom: Wasserstein-2 distance between E-SINDy and Bayesian-SINDy with Spike-and-slab prior. 
    (b) Exponential convergence for E-SINDy in terms of False Discovery Probability and True Discovery Probability for the synthetic Lotka-volterra dataset. }
    \label{fig:conv_and_uq}
\end{figure*}

From the other side, it is also very challenging to characterize the effect of Bootstrap applying on a sparse variable selection procedure. In general, Bootstrapping is a computational method to improve inference on small samples using the idea of resampling~\citep{efron1979computers,hall2013bootstrap,efron1994introduction}. 
% The consistency of the Bootstrap procedure is shown in~\citep{bickel1983bootstrapping}. 
The residual-bootstrap LASSO is inconsistent for sparse models~\citep{chatterjee2011bootstrapping}, but the residual-bootstrap distribution of Adaptive LASSO~\citep{zou2006adaptive} is consistent. 
Resampling methods could help to improve variable selection performance for LASSO~\citep{bach2008bolasso,meinshausen2010stability,werner2022loss}, but there has been a limited study that jointly considers Bootstrapping and TLSE. Even though Giurcanu shows the consistency of residual-Bootstrap the TLSE estimators in~\citep{giurcanu2016thresholding}, to the best of our knowledge, the detailed interaction between Bootstrap and TLSE still remains unknown, which set back our understanding on the remarkable performance of E-SINDy. 





% \begin{figure*}
%     \includegraphics[width=\textwidth]{paper/figs/exp_converge_fig2.pdf}
%     \caption{(a) We observe exponential convergence for Bagging inclusion probability TLSE of Empirical False Discovery Probability (EFDP) and Empirical True Discovery Probability (ETDP). As stated in informal theorem, we set $g_1(p,q)=1, \alpha_1(p_c)=2\cdot p_c, b_1=4$ and $g_2(q)=\sqrt{\frac{q}{3}}, \alpha_2(p_c)=\frac{20p_c^2}{9}-\frac{2p_c}{3}+0.05, b_2=0$. (b) Following similar settings in (a) with governing equation discovery based structure. Lotka model has four active coefficients and extended Lotka model has eight active coefficients. For both models with different sparsity levels, we observe exponential convergence. }
%     \label{fig:exp_convergence}
% \end{figure*}

To establish the theoretical understanding, we investigate the bootstrap aggregating inclusion probability based Thresholding Least-Squares Estimation as an ensembling technique for sparse linear regression and uncertainty quantification. 
% We provide a comprehensive discussion of the theory of E-SINDy, including its effectiveness in variable selection, validity in uncertainty quantification, and efficiency in computation. 
Through concentration probability bounds, we show the oracle property in Thm.~\ref{thm:oracle_property} of bootstrapping inclusion probability TLSE with an exponential convergence rate under milder regularity conditions, which explains the empirically observed exponential convergence of error bounds in (like in Fig.~\ref{fig:conv_and_uq} (b)). The following informal version of our main
result that clarifies the exponential rate of convergence for both FDP and TDP.
In our formal Theorem \ref{thm:oracle_property}, we show a qualitative result that captures this exponential behavior in the informal theorem. 
% We note here the bounds in the formal Theorem are relatively loose when the sample size is small due to the union bound to the model size (c.f. Appendix~\ref{app:proof_theorem}). 
% Despite in practice, as shown in Fig.~\ref{fig:conv_and_uq} (b), the exponential convergence can act sublinearly to the model size, it is technically hard in theory to exactly quantify this sublinear behavior from Binomial trails. 
% We present the Informal Theorem in the following and defer the discussion related to the tightness of the bound in Sec.~\ref{sec:discussion}.  


\begin{extthm}[Theorem (Informal)]
    Let $n$ be the number of samples, $p$ be the model size, and $q$ be the number of active indices. The false discovery probability of sparse set estimation of bagging inclusion probability TLSE satisfies 
    \begin{align}
        FDP \leq g_1(p,q)\exp\lrp{-\alpha_1(p_c)n+b_1}.
    \end{align}
    The true discovery probability of sparse set estimation of bagging inclusion probability TLSE satisfies 
    \begin{align}
        TDP \leq g_2(q)\exp\lrp{-\alpha_2(p_c)n+b_2},
    \end{align}
    where $g_1(\cdot),g_2(\cdot),\alpha_1(\cdot),\alpha_2(\cdot)$ are some functions and $b_1,b_2$ are some constants. 
\end{extthm}


Besides the oracle property for variable selection, we examine that the E-SINDy algorithm with bagging inclusion probability based TLSE is valid for uncertainty quantification (UQ) in Lemma~\ref{lem:uq_BIP}. We show the similarity between bagging inclusion probability TLSE and Bayesian UQ methods with Spike-and-slab prior in~\citep{ishwaran2005spike,hirsh2022sparsifying} from (i) approximate Bayesian inference with Weighted Likelihood Bootstrap~\citep{newton1994approximate} and (ii) Bayesian Bootstrap Spike-and-Slab LASSO~\citep{nie2022bayesian}. 
Compared to Bayesian UQ methods, Bootstrapping based methods could provide similar uncertainty estimate, but are much more computationally efficient. For example, in the Lotka-Volterra model discovery, Bayesian SINDy reuqires an execution for more than 12 hours while E-SINDy takes less than 20 seconds. We correspondingly discuss the difference in computational complexity between Bayesian MCMC and bagging inclusion probability-based methods in Remark~\ref{rem:computation}.

In Fig.~\ref{fig:conv_and_uq} (a) top, we show the effectiveness of E-SINDy for distributional convergence and uncertainty quantification. E-SINDy algorithm quickly converges to the true mean with an increasing number of samples, and generates an uncertainty estimate around the true value. In Fig.~\ref{fig:conv_and_uq} (a) bottom, the blue solid line represents the average Wasserstein-2 distance over ten experimental trials. 
The shaded area shows the confidence interval estimate using the $80\%$ percentile over the ten trials. 
The distributional estimation of E-SINDy converges to the estimation of Bayesian SINDy with large sample sizes. We discuss the connection between E-SINDy and Bayesian MCMC in Sec.~\ref{sec:connection_bayesian}, and show the validity for uncertainty quantification in Lemma~\ref{lem:uq_BIP}.
In Fig.~\ref{fig:conv_and_uq} (b), we plot the convergence of the empirical false discovery probability (FDP) and the empirical true discovery probability (TDP). 
As stated in the Informal Theorem, the exponential error bound holds with $g_1(p,q)=1, \alpha_1(p_c)=p_c, b_1=4/3$ and $g_2(q)=\sqrt{\frac{q}{2}}, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{20}, b_2=0$. 
% The inferential procedure of E-SINDy is able to (i) accelerate the sparse inference process with smaller sample sizes and (ii) perform valid uncertainty quantification. 

% TODO-1
We further apply bagging inclusion probability based TLSE into broader scenarios, from synthetic sparse linear regression to physics model discovery. 
From the simulation of sparse linear regression under different settings, we observe an accelerated effect of bagging inclusion probability based variable selection in terms of the sample size. Additionally, we perform an experimental study on the robustness of hyperparameters in varying experimental settings for bagging inclusion probability based TLSE and other baseline methods. The bagging inclusion probability based TLSE has very stable performances with respect to changes in sparsity and noise levels. 
For governing equation discovery, we observe the E-SINDy based algorithm, could perform correct variable selection and uncertainty quantification. The estimation bias quickly reduces with more observation points and the uncertainty estimation is valid under noisy settings. This experimental study, as the supplement of Lem.~\ref{lem:uq_BIP}, show that the E-SINDy with bagging inclusion probability based TLSE uncertainty quantification is valid, which is functionally equivalent to Bayesian MCMC with sparsifying priors~\citep{hirsh2022sparsifying}. 

The contribution of this paper is threefold: 


% The sparsity of LASSO is promoted from a $\ell_1$ constraint as a relaxation of a non-convex $\ell_0$ minimization problem. 
% In this work, we propose Bootstrap Thresholding Least-square estimator (TLSE) to 

% \begin{itemize}
%     % \item Governing equation, why important, and hard to solve... 
    
    

%  \item There has been an extensive discussion in the development of theory and algorithm for sparse regression. 
% One of the most popular methods is the Least Absolute Shrinkage and Selection Operator (LASSO)~\citep{tibshirani1996regression}. LASSO good for (statistical property...). However, LASSO might not work for ... 
%   \item Challenges/open Qs. 
  
%   \item Gap we filled in for this paper. [E-Sindy/Thresholding LSq]  
%   % it simply works -> we show why it works -> we compare existing (bayesian) methods

%  \item In this paper, we propose a bootstrapping based thresholding least-squares estimator for sparse linear regression and variable selection problems. Thresholding regression methods are widely used in many problems like wavelet regression~\citep{donoho1994ideal}, denoising~\citep{donoho1995noising}, robust high-dimensional regression~\citep{bhatia2015robust}, and sparse identification of physical systems~\citep{brunton2016discovering}. 

%  \item Alternatively, a thresholding strategy has been... 

% In this paper, we propose... 

% \end{itemize}

\begin{enumerate}
    \item We study the theoretical extension of E-SINDy algorithm with bagging inclusion probability TLSE and analyze its oracle property under mild regularity conditions with an exponential convergence rate. 
    \item We show that bagging inclusion probability TLSE is computationally efficient compared to Bayesian methods, and could perform valid uncertainty quantification with guarantee in an asymptotic sense. 
    \item We implement and verify the effect of bagging inclusion probability TLSE in both synthetic sparse linear regression setting and physical equation discovery. We verify the effect of accelerated variable selection as well as the validity in uncertainty quantification. 
\end{enumerate}

In the following sections, we first perform the background study on SINDy algorithm and variable selection methods in Sec.~\ref{sec:background}. Then, we review the analysis on Thresholding Least-square estimation in Sec.~\ref{sec:tlse} and propose theoretical analysis for E-SINDy with bootstrapping inclusion probability based TLSE in Sec.~\ref{sec:bs_tlse}. We finally conduct various experiments on sparse linear regression and sparse physics model discovery in Sec.~\ref{sec:simulation}. 

==> intro2.tex <==
Governing equation discovery is essential for physical science. In the modern era of big data, an incredible amount of data gives rise to opportunities to perform data-driven model discovery~\citep{schmidt2009distilling} based on the first principle, which is widely applicable for scientific problems including neuroscience, epidemiology, astronomy, robotics, and so on. 
Even if there have been many discussions about model discovery algorithms, sparse regression methods are one of the most popular methods due to their simplicity in implementation, efficiency in computation, and robustness in accuracy.
The sparse identification of nonlinear dynamics algorithm (SINDy)~\citep{brunton2016discovering} utilizes sequential Thresholding Least-square Estimator (TLSE) to promote sparsity. 
More recently, Fasel et al.~\citep{fasel2022ensemble} propose Ensemble SINDy (E-SINDy) which constructs bootstrap replicates based on the TLSE-based variable selection. With the Bootstrapping step, E-SINDy not only enables uncertainty quantification in parametric inference, but also improves the robustness of variable selection under limited and noisy data. Both SINDy and E-SINDy algorithms achieve huge success from the engineering perspective. 

% \begin{figure*}
%     \includegraphics[width=0.95\textwidth]{paper/figs/informal_Thm_1.pdf}
%     \caption{We observe exponential convergence for Bagging inclusion probability TLSE of Empirical False Discovery Probability (EFDP) and Empirical True Discovery Probability (ETDP). The orange curve is a dominated by $\exp(-\alpha\cdot n)$ where $\alpha$ is a constant. } 
%     \label{fig:informal_thm1}
% \end{figure*}



From the theoretical side, both SINDy and Bootstrapped SINDy are nontrivial to be understood. From the standpoint of variable selection, most statistical literature focuses on the least absolute shrinkage and selection operator (LASSO)~\citep{tibshirani1996regression}. The statistical properties of LASSO-based methods have been systematically studied, including the consistency~\citep{zhao2006model}, the oracle property in classic regression settings~\citep{fan2001variable,zou2006adaptive}, and in high-dimensional settings~\citep{wainwright2019high,huang2008asymptotic}. 
Even if thresholding-based methods achieve good performances in many problems~\citep{donoho1994ideal,donoho1995noising,bhatia2015robust}, the development of its statistical foundation is not as good as the LASSO. 
Until recently, Giurcanu propose a statistical understanding of thresholding-based estimators~\citep{giurcanu2016thresholding}, and show similar statistical properties of the thresholding-based estimatior to the LASSO. 

% Exchange a <-> b
% TDP CAP not consistetn
\begin{figure*}[!ht]
    \includegraphics[width=\textwidth]{paper/figs/Fig1_revised.pdf}
    \caption{(a) Top: evolution of distributional estimation of the E-SINDy algorithm over different sample sizes. The inference of the E-SINDy algorithm quickly converges to a delta measure centered around the true value. Bottom: Wasserstein-2 distance between E-SINDy and Bayesian-SINDy with Spike-and-slab prior. 
    The blue solid line represents the average Wasserstein-2 distance over ten trials. 
    The shaded area shows the confidence interval estimate using the $80\%$ percentile over the ten trials. 
    The distributional estimation of E-SINDy converges to the estimation of Bayesian SINDy with large sample sizes. We discuss the connection between E-SINDy and Bayesian MCMC in Sec.~\ref{sec:connection_bayesian}, and show the validity for uncertainty quantification in Lemma~\ref{lem:uq_BIP}. (b) Exponential convergence for E-SINDy in terms of Empirical False Discovery Probability~\eqref{def:FDP} and True Discovery Probability~\eqref{def:TDP} defined for the synthetic Lotka-volterra dataset. As stated in the Informal Theorem, the exponential error bound holds with $g_1(p,q)=1, \alpha_1(p_c)=p_c, b_1=4/3$ and $g_2(q)=\sqrt{\frac{q}{2}}, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{20}, b_2=0$. Our main Theorem~\ref{thm:oracle_property} captures this behavior under relatively large sample sizes. }
    \label{fig:conv_and_uq}
\end{figure*}

In addition, it is difficult to characterize a Bootstrapping-based sparse variable selection procedure. In general, Bootstrapping is a computational method to improve inference on small samples using the idea of resampling~\citep{efron1979computers,hall2013bootstrap,efron1994introduction}. 
% The consistency of the Bootstrap procedure is shown in~\citep{bickel1983bootstrapping}. 
The residual-bootstrap LASSO is inconsistent for sparse models~\citep{chatterjee2011bootstrapping}, but the residual-bootstrap distribution of Adaptive LASSO~\citep{zou2006adaptive} is consistent. 
Resampling methods could help to improve variable selection performance for LASSO~\citep{bach2008bolasso,meinshausen2010stability,werner2022loss}, but there has been a limited study that jointly considers Bootstrapping and TLSE. Even though Giurcanu shows the consistency of residual-Bootstrap the TLSE estimators in~\citep{giurcanu2016thresholding}, to the best of our knowledge, the detailed interaction between Bootstrap and TLSE still remains unknown, which set back our understanding on the remarkable performance of E-SINDy. 





% \begin{figure*}
%     \includegraphics[width=\textwidth]{paper/figs/exp_converge_fig2.pdf}
%     \caption{(a) We observe exponential convergence for Bagging inclusion probability TLSE of Empirical False Discovery Probability (EFDP) and Empirical True Discovery Probability (ETDP). As stated in informal theorem, we set $g_1(p,q)=1, \alpha_1(p_c)=2\cdot p_c, b_1=4$ and $g_2(q)=\sqrt{\frac{q}{3}}, \alpha_2(p_c)=\frac{20p_c^2}{9}-\frac{2p_c}{3}+0.05, b_2=0$. (b) Following similar settings in (a) with governing equation discovery based structure. Lotka model has four active coefficients and extended Lotka model has eight active coefficients. For both models with different sparsity levels, we observe exponential convergence. }
%     \label{fig:exp_convergence}
% \end{figure*}

In this paper, to establish a theoretical understanding, we investigate Bootstrap Inclusion Probability (BIP) based Thresholding Least-Squares Estimation as an ensembling technique for sparse linear regression and variable selection. We provide a comprehensive discussion of Bootstrapping based TLSE, including its effectiveness in variable selection, validity in uncertainty quantification, and efficiency in computation. We aim to fill in this gap in the literature with a systematic study of Bootstrapping, ensembling and Thresholding-based estimators for sparse regression. 
We first review the theoretical foundation of TLSE in~\citep{giurcanu2016thresholding}. Then, we establish Bootstrap inclusion probability (BIP) TLSE based variable selection in Alg.~\ref{alg:bag_tlse}. 
Stepping further from BIP TLSE, we incorporate the out-of-bag (OOB) error to reweight the averaging of inclusion probability process in Alg.~\ref{alg:bag_tlse_oob}, which generally achieves the best. 


Through concentration probability bounds, we show the oracle property in Thm.~\ref{thm:oracle_property} of Bootstrapped TLSE with an exponential convergence rate under milder regularity conditions, which explains the exponential convergence of error bounds in Fig.~\ref{fig:conv_and_uq} (b). The following informal version of our main
result that clarifies the rate of convergence.
In our formal Theorem \ref{thm:oracle_property}, we show a qualitative result that characterizes the convergence rate is exponential for both False Discovery Probability (FDP) and True Discovery Probability (TDP). 
We note here the bounds in the formal Theorem are relatively loose when the sample size is small due to the union bound to the model size (c.f. Appendix~\ref{app:proof_theorem}). 
Despite in practice, as shown in Fig.~\ref{fig:conv_and_uq} (b), the exponential convergence can act sublinearly to the model size, it is technically hard in theory to exactly quantify this sublinear behavior from Binomial trails. 
We present the Informal Theorem in the following and defer the discussion related to the tightness of the bound in Sec.~\ref{sec:discussion}.  


\begin{extthm}[Theorem (Informal)]
    Let $n$ be the number of samples, $p$ be the model size, and $q$ be the number of active indices. The false discovery probability of sparse set estimation of BIP TLSE satisfies 
    \begin{align}
        FDP \leq g_1(p,q)\exp\lrp{-\alpha_1(p_c)n+b_1}.
    \end{align}
    The true discovery probability of sparse set estimation of BIP TLSE satisfies 
    \begin{align}
        TDP \leq g_2(q)\exp\lrp{-\alpha_2(p_c)n+b_2},
    \end{align}
    where $g_1(\cdot),g_2(\cdot),\alpha_1(\cdot),\alpha_2(\cdot)$ are some functions and $b_1,b_2$ are some constants. 
\end{extthm}

To illustrate the effect of E-SINDy and general Bootstrapping TLSE, we present two scenarios in the following. 
In Fig.~\ref{fig:conv_and_uq} (a) top, we show the effectiveness of E-SINDy for distributional convergence and uncertainty quantification. E-SINDy algorithm quickly converges to the true mean with an increasing number of samples, and generates an uncertainty estimate around the true value. 
In Fig.~\ref{fig:conv_and_uq} (b), we plot the convergence of the empirical false discovery probability (FDP) and the empirical true discovery probability (TDP). It is observable that with an increasing number of samples, both error curves decay very fast that could be bounded by an exponential function.  
Besides, as shown in Fig.~\ref{fig:conv_and_uq} (a) bottom, the distributional estimation of E-SINDy and the distributional estimation of Bayesian SINDy via Spike-and-slab prior empirically converge to each other from the Wasserstein-2 distance plot. 
From all these observations, we believe the inferential procedure of E-SINDy is able to (i) accelerate the sparse inference process with smaller sample sizes and (ii) perform valid uncertainty quantification. These observations motivate us to study the behavior of Bootstrapped thresholding least-squares estimator in theory. 


Besides the oracle property for variable selection, we examine that the BIP TLSE algorithm is valid for uncertainty quantification (UQ) in Lemma~\ref{lem:uq_BIP}. We show the similarity between BIP TLSE and Bayesian UQ methods with Spike-and-slab prior in~\citep{hirsh2022sparsifying} from (a) approximate Bayesian inference with Weighted Likelihood Bootstrap~\citep{newton1994approximate} and (b) Bayesian Bootstrap Spike-and-Slab LASSO~\citep{nie2022bayesian}. 
Compared to Bayesian UQ methods, Bootstrapping based methods could provide similar uncertainty estimate, but are much more computationally efficient. For example, in the Lotka-Volterra model discovery, Bayesian SINDy reuqires an execution for more than 12 hours while E-SINDy takes less than 20 seconds. We correspondingly discuss the difference in computational complexity between Bayesian MCMC and BIP-based methods in Remark~\ref{rem:computation}.

% TODO-1
In the experiments, we apply BIP selection to various cases, including synthetic linear regression and physical data discovery. 
From the simulation of sparse linear regression under different settings, we observe an accelerated effect of BIP variable selection in terms of the sample size. Additionally, we perform an experimental study on the robustness of hyperparameters in varying experimental settings for BIP and other baseline methods. The BIP TLSE estimator has very stable performances with respect to changes in sparsity and noise levels. 
For governing equation discovery, we observe BIP TLSE-based algorithm (or equivalently E-SINDy), could perform correct variable selection and uncertainty quantification. The estimation bias quickly reduces with more observation points and the uncertainty estimation is valid under noisy settings. This experimental study, as the supplement of Lem.~\ref{lem:uq_BIP}, show that the BIP TLSE-based uncertainty quantification is valid, which is functionally equivalent to Bayesian MCMC with sparsifying priors~\citep{hirsh2022sparsifying}. 

The contribution of this paper is threefold: 


% The sparsity of LASSO is promoted from a $\ell_1$ constraint as a relaxation of a non-convex $\ell_0$ minimization problem. 
% In this work, we propose Bootstrap Thresholding Least-square estimator (TLSE) to 

% \begin{itemize}
%     % \item Governing equation, why important, and hard to solve... 
    
    

%  \item There has been an extensive discussion in the development of theory and algorithm for sparse regression. 
% One of the most popular methods is the Least Absolute Shrinkage and Selection Operator (LASSO)~\citep{tibshirani1996regression}. LASSO good for (statistical property...). However, LASSO might not work for ... 
%   \item Challenges/open Qs. 
  
%   \item Gap we filled in for this paper. [E-Sindy/Thresholding LSq]  
%   % it simply works -> we show why it works -> we compare existing (bayesian) methods

%  \item In this paper, we propose a bootstrapping based thresholding least-squares estimator for sparse linear regression and variable selection problems. Thresholding regression methods are widely used in many problems like wavelet regression~\citep{donoho1994ideal}, denoising~\citep{donoho1995noising}, robust high-dimensional regression~\citep{bhatia2015robust}, and sparse identification of physical systems~\citep{brunton2016discovering}. 

%  \item Alternatively, a thresholding strategy has been... 

% In this paper, we propose... 

% \end{itemize}

\begin{enumerate}
    \item Motivated from the Ensemble SINDy procedure, we propose BIP TLSE algorithm and analyze its oracle property under mild regularity conditions with an exponential convergence rate. 
    \item We show that BIP TLSE is computationally efficient compared to Bayesian methods, and could perform uncertainty quantification with guarantee in an asymptotic sense. 
    \item We implement and verify the effect of BIP TLSE in both synthetic sparse linear regression setting and physical equation discovery. We verify the effect of accelerated variable selection as well as the validity in uncertainty quantification. 
\end{enumerate}

In the following sections, we first perform a background study on SINDy algorithm and variable selection methods in Sec.~\ref{sec:background}. Then, we review the analysis on Thresholding Least-square estimation in Sec.~\ref{sec:tlse} and propose theoretical analysis for E-SINDy in Sec.~\ref{sec:bs_tlse}. We perform experimental study on sparse linear regression and sparse physics model discovery in Sec.~\ref{sec:simulation}. 

==> intro3_backup.tex <==

Data-driven model discovery methods based on sparse linear regression are promising, because they enable discovering
interpretable and generalizable models that balance accuracy and efficiency. The sparse identification of nonlinear dynamics (SINDy) algorithm~\citep{brunton2016discovering} promotes sparsity using the sequential thresholding least-squares (STLS) estimator.  Recently, SINDy was extended to incorporate ensembling techniques, leveraging bootstrap aggregating (bagging) methods to produce the robust and computationally efficient probabilistic model discovery method E-SINDy~\citep{fasel2022ensemble}. With the bootstrapping step, E-SINDy empirically improves the robustness of variable selection under limited and noisy data, and enables uncertainty quantification in parametric inference. 
% Even if E-SINDy algorithms achieve huge success from the engineering perspective, a theoretical understanding is missing to explain the improvements. 
In this paper, we study sparse linear regression using bagging inclusion probability based STLS estimation, a generalization of the sparse regression algorithm used in E-SINDy. We prove that the E-SINDy algorithm is able to perform correct sparse model identification with exponential convergence in terms of false discovery probability (FDP) and true discovery probability (TDP). The theoretical result on the correct sparse identification additionally offers a statistical guarantee on the uncertainty quantification of E-SINDy. These theoretical results reveal the effectiveness of E-SINDy for sparse model discovery, and its potential as a general sparse linear regression method. 


%From the standpoint of variable selection, it is nontrivial to derive the theoretical guarantee of SINDy and E-SINDy as thresholding procedures. Most literature alternatively focuses on the least absolute shrinkage and selection operator (LASSO)~\citep{tibshirani1996regression} which utilizes an $\ell_1$ shrinkage estimator for sparse regression. The statistical properties of LASSO-based methods have been systematically studied, including the consistency~\citep{zhao2006model}, the oracle property in classic regression settings~\citep{fan2001variable,zou2006adaptive}, and in high-dimensional settings~\citep{wainwright2019high,huang2008asymptotic}. 
%From the Bayesian perspective, a hierarchical Bayesian model with Spike-and-slab~\citep{mitchell1988bayesian,george1997approaches,ishwaran2005spike} or regularized horseshoe prior~\citep{carvalho2009handling,carvalho2010horseshoe} are thoroughly studied with the effectiveness for Bayesian sparse inference.  %Even if thresholding-based methods achieve good performances in many problems~\citep{donoho1994ideal,donoho1995noising,bhatia2015robust}, the development of its statistical foundation is not fully established. 
%Only until recently, Giurcanu propose a statistical understanding of thresholding-based estimators~\citep{giurcanu2016thresholding}, and show statistical guarantees of the thresholding-based estimatior in sparse variable selection.

Variable selection and sparse regression have a rich history in data science and statistics. In classical theory, the likelihood ratio test is one of the earliest variable selection methods~\citep{wilks1938large}. More recently, the least absolute shrinkage and selection operator (LASSO) uses an $\ell_1$ shrinkage estimator for sparse inference~\citep{tibshirani1996regression}. 
%Knight and Fu~\citep{fu2000asymptotics} showed the asymptotic behavior of LASSO type estimators. 
%Zhao and Yu~\citep{zhao2006model} proved the consistency of LASSO given the Irrepresentable Condition.
%Later on, Fan and Li~\citep{fan2001variable} proposed a penalized least square method with smoothly clipped absolute deviation (SVAD) with oracle property. 
%Zou proposed an adaptive LASSO procedure that utilizes an ordinary least-square adjusted $\ell_1$ penalty with consistency and the oracle property~\citep{zou2006adaptive}.  
%Park and Casella considered the Bayesian formulation of LASSO with a Laplace prior in~\citep{park2008bayesian}. 
%In high-dimensional settings, LASSO could perform consistent variable selection under Lower eigenvalue and  Mutual incoherence conditions ~\citep{wainwright2009sharp,wainwright2019high}. 
The statistical properties of LASSO-based methods have been systematically studied, including the asymptotic behavior~\citep{fu2000asymptotics}, consistency~\citep{zhao2006model}, the oracle property in classic regression settings~\citep{fan2001variable,zou2006adaptive}, and in high-dimensional settings~\citep{wainwright2009sharp,wainwright2019high,huang2008asymptotic}. 
From the Bayesian perspective, a hierarchical Bayesian model with spike-and-slab~\citep{mitchell1988bayesian,george1997approaches,ishwaran2005spike}, Laplace~\citep{park2008bayesian}, or regularized horseshoe prior~\citep{carvalho2009handling,carvalho2010horseshoe} are thoroughly studied with the effectiveness for Bayesian sparse inference. 
For thresholding-based estimators, even if these estimators have been widely applied in problems like wavelet regression~\citep{donoho1994ideal}, denoising~\citep{donoho1995noising}, robust high-dimensional regression~\citep{bhatia2015robust}, and sparse identification of physical systems~\citep{brunton2016discovering}, the development of their statistical foundation is not fully established. The first work on statistical guarantees for STLS based estimators investigated the oracle property of STLS estimators in low- and high-dimensional settings, and showed the consistency of residual-bootstrap for STLS estimators~\citep{giurcanu2016thresholding}. 
%
Characterizing the effect of bootstrapping applied to sparse variable selection adds another layer of complexity. 
%
In general, bootstrapping is a computational method to improve inference on small samples using the idea of resampling~\citep{efron1979computers,hall2013bootstrap,efron1994introduction}. The residual-bootstrap LASSO is inconsistent for sparse models~\citep{chatterjee2011bootstrapping}, but the residual-bootstrap distribution of Adaptive LASSO~\citep{zou2006adaptive} is consistent. Resampling methods could help to improve variable selection performance for LASSO~\citep{bach2008bolasso,meinshausen2010stability,werner2022loss}, but there has only been limited studies that jointly consider bootstrapping and STLS. To the best of our knowledge, the detailed interaction between bootstrap and STLS still remains unknown. 


\begin{figure*}[t]
    \includegraphics[width=\textwidth]{paper/figs/Fig1_revised.pdf}
    \caption{(a) Top: convergence of distributional estimation of the Bayesian SINDy and E-SINDy algorithm over different sample sizes. Bottom: Wasserstein-2 distance between E-SINDy and Bayesian-SINDy with Spike-and-slab prior. 
    (b) Exponential convergence for E-SINDy in terms of False Discovery Probability and True Discovery Probability for the synthetic Lotka-Volterra dataset. 
    % The exponential error bound holds with $g_1(p,q)=1, \alpha_1(p_c)=p_c, b_1=4/3$ and $g_2(q)=\sqrt{\frac{q}{2}}, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{20}, b_2=0$, as stated in the informal theorem. 
    }
    \label{fig:conv_and_uq}
\end{figure*}

%From the other side, it is also very challenging to characterize the effect of Bootstrap applying on a sparse variable selection procedure. In general, Bootstrapping is a computational method to improve inference on small samples using the idea of resampling~\citep{efron1979computers,hall2013bootstrap,efron1994introduction}. 
% The consistency of the Bootstrap procedure is shown in~\citep{bickel1983bootstrapping}. 
%The residual-bootstrap LASSO is inconsistent for sparse models~\citep{chatterjee2011bootstrapping}, but the residual-bootstrap distribution of Adaptive LASSO~\citep{zou2006adaptive} is consistent. 
%Resampling methods could help to improve variable selection performance for LASSO~\citep{bach2008bolasso,meinshausen2010stability,werner2022loss}, but there has been a limited study that jointly considers Bootstrapping and TLSE. Even though Giurcanu shows the consistency of residual-Bootstrap the TLSE estimators in~\citep{giurcanu2016thresholding}, to the best of our knowledge, the detailed interaction between Bootstrap and TLSE still remains unknown, which set back our understanding on the remarkable performance of E-SINDy. 



To establish the theoretical understanding of the interaction between bootstrapping and STLS, we investigate the bootstrap aggregating inclusion probability based STLS estimation. % as an ensembling technique for sparse linear regression and uncertainty quantification. 
% We provide a comprehensive discussion of the theory of E-SINDy, including its effectiveness in variable selection, validity in uncertainty quantification, and efficiency in computation. 
Through concentration probability bounds, we show the oracle property in Thm.~\ref{thm:oracle_property} of bootstrapping inclusion probability STLS with an exponential convergence rate under milder regularity conditions. 
%
This theoretical result guarantees that the bootstrapping inclusion probability STLS could always perform correct model identification (or variable selection?) when having sufficiently large sample sizes. 
%
In Fig.~\ref{fig:conv_and_uq} (b), the exponential convergence of error bounds and the empirical convergence using E-SINDy for the FDP and TDP are shown. 
%which explains the empirically observed exponential convergence of error bounds in (like in Fig.~\ref{fig:conv_and_uq} (b)). 
A generalized theorem in the following captures an overall exponential convergence behavior for both FDP and TDP as indicated in Fig.~\ref{fig:conv_and_uq} (b).
% In our formal Theorem \ref{thm:oracle_property}, we show a qualitative result that captures the exponential behavior in the informal theorem (this sentence is a bit unclear?). 
% We note here the bounds in the formal Theorem are relatively loose when the sample size is small due to the union bound to the model size (c.f. Appendix~\ref{app:proof_theorem}). 
% Despite in practice, as shown in Fig.~\ref{fig:conv_and_uq} (b), the exponential convergence can act sublinearly to the model size, it is technically hard in theory to exactly quantify this sublinear behavior from Binomial trails. 
% We present the Informal Theorem in the following and defer the discussion related to the tightness of the bound in Sec.~\ref{sec:discussion}.  


\begin{extthm}[Main Theorem (Generalized)]
    Let $n$ be the number of samples, $p$ be the model size, and $q$ be the number of non-sparse indices. The false discovery probability of sparse set estimation of bagging inclusion probability STLS satisfies 
    \begin{align}
        FDP \leq g_1(p,q)\exp\lrp{-\alpha_1(p_c)n+b_1}=\mathcal{O}\lrp{\exp\lrp{-n}}.
    \end{align}
    The true discovery probability of sparse set estimation of bagging inclusion probability STLS satisfies 
    \begin{align}
        TDP \geq 1-g_2(q)\exp\lrp{-\alpha_2(p_c)n+b_2}=1-\mathcal{O}\lrp{\exp\lrp{-n}},
    \end{align}
    where $g_1(\cdot),g_2(\cdot),\alpha_1(\cdot),\alpha_2(\cdot)$ are some functions and $b_1,b_2$ are some constants. 
\end{extthm}

\vspace{10pt}

\noindent In Thm.~\ref{thm:oracle_property}, we demonstrate a proof by setting $g_1(p,q)=p-q, \alpha_1(p_c)=\frac{p_c}{3}, b_1=1/3$ and $g_2(q)=q, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{6}, b_2=0$. In empirical studies, this bound could be even tighter by setting $g_1(p,q)=1, \alpha_1(p_c)=p_c, b_1=4/3$ and $g_2(q)=\sqrt{\frac{q}{2}}, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{20}, b_2=0$, which corresponds to the red curves in Fig.~\ref{fig:conv_and_uq} (b). 


Besides the oracle property for variable selection, we examine that the E-SINDy algorithm with bagging inclusion probability based STLS estimator is valid for uncertainty quantification (UQ) in Lemma~\ref{lem:uq_BIP}. We show the similarity between bagging inclusion probability STLS and Bayesian UQ methods with spike-and-slab prior in~\citep{ishwaran2005spike,hirsh2022sparsifying} from (i) approximate Bayesian inference with Weighted Likelihood Bootstrap~\citep{newton1994approximate} and (ii) Bayesian Bootstrap Spike-and-Slab LASSO~\citep{nie2022bayesian}. 
%
Compared to Bayesian UQ methods, bootstrapping based methods could provide similar uncertainty estimate, but are computationally much more efficient. For example, in the Lotka-Volterra model discovery, Bayesian SINDy requires an execution of more than 12 hours, while E-SINDy takes less than 20 seconds. We correspondingly discuss the difference in computational complexity between Bayesian MCMC and bagging inclusion probability-based methods in Remark~\ref{rem:computation}. 
%
The effectiveness of E-SINDy for distributional convergence and uncertainty quantification is shown in Fig.~\ref{fig:conv_and_uq} (a) top. The E-SINDy algorithm quickly converges to the true mean with an increasing number of samples, and generates an uncertainty estimate around the true value. In Fig.~\ref{fig:conv_and_uq} (a) bottom, the blue solid line represents the average Wasserstein-2 distance over ten experimental trials. The shaded area shows the confidence interval estimate using the $80\%$ percentile over the ten trials. The distributional estimation of E-SINDy converges to the estimation of Bayesian SINDy with large sample sizes. We discuss the connection between E-SINDy and Bayesian MCMC in Sec.~\ref{sec:connection_bayesian}, and show the validity for uncertainty quantification in Lemma~\ref{lem:uq_BIP}.


%In Fig.~\ref{fig:conv_and_uq} (b), we plot the convergence of the empirical false discovery probability (FDP) and the empirical true discovery probability (TDP). As stated in the Informal Theorem, the exponential error bound holds with $g_1(p,q)=1, \alpha_1(p_c)=p_c, b_1=4/3$ and $g_2(q)=\sqrt{\frac{q}{2}}, \alpha_2(p_c)=\frac{(1-2 p_c)^2}{20}, b_2=0$. 

% The inferential procedure of E-SINDy is able to (i) accelerate the sparse inference process with smaller sample sizes and (ii) perform valid uncertainty quantification. 

We further apply bagging inclusion probability based STLS to broader scenarios, from synthetic sparse linear regression to physics model discovery. From the simulation of sparse linear regression under different settings, we observe an accelerated effect of bagging inclusion probability based variable selection in terms of the sample size. Additionally, we perform an experimental study on the robustness of hyperparameters in varying experimental settings for bagging inclusion probability based STLS and other baseline methods. The bagging inclusion probability based STLS has very stable performances with respect to changes in sparsity and noise levels. 
For governing equation discovery, we observe that the E-SINDy based algorithm can perform correct variable selection and uncertainty quantification. The estimation bias quickly reduces with more observation points and the uncertainty estimation is valid under noisy settings. The experimental study, as the supplement of Lem.~\ref{lem:uq_BIP}, shows that the E-SINDy with bagging inclusion probability based STLS uncertainty quantification is valid, which is functionally equivalent to Bayesian MCMC with sparsifying priors~\citep{hirsh2022sparsifying}. 

The contribution of this paper is threefold: 



\begin{enumerate}
    \item We study the theoretical extension of E-SINDy algorithm with bagging inclusion probability STLS and analyze its oracle property under mild regularity conditions with an exponential convergence rate. 
    \item We show that bagging inclusion probability STLS is computationally efficient compared to Bayesian methods, and can perform valid uncertainty quantification with guarantee in an asymptotic sense. 
    \item We implement and verify the effect of bagging inclusion probability STLS in both synthetic sparse linear regression setting and physical equation discovery. We verify the effect of accelerated variable selection as well as the validity in uncertainty quantification. 
\end{enumerate}

In the following, we first introduce the SINDy algorithm and variable selection methods in Sec.~\ref{sec:background}. Then, we review the analysis on sequential thresholding least-squares estimation in Sec.~\ref{sec:tlse}, and propose theoretical analysis for E-SINDy with bootstrapping inclusion probability based STLS in Sec.~\ref{sec:bs_tlse}. We finally conduct various experiments on sparse linear regression and sparse physics model discovery in Sec.~\ref{sec:simulation}. 

==> naive_bs.tex <==
In a general sense, Bootstrapping allows the variance estimate around the sample mean. Therefore, it enlarges the variance term for OLS. The effect of Bootstrapping TLSE mean would be the OLS estimate.Additionally,  OLS is Best Linear Unbiased Estimator (BLUE), so the linear combination of OLS will be sub-optimal comparing to the BLUE. We construct the naive bagging OLS estimator in the following way: 

Suppose we have $n$ bootstrap replicates with OLS indexed by $\{\bar\beta^b\}_{b=1}^n$. Consider an estimator of $\hat K$ that
\begin{align}
    \label{eqn:K_bag_def}
    \hat K_{bag} = \left\{j\in I: \left|\frac{1}{n}\sum_{b=1}^n \bar\beta^b_j \right| \leq \sigma\sqrt{2\log(1/\delta)(X_j^TX_j)^{-1}}\right\}. 
\end{align}

% Notice from~\eqref{eqn:K_bag_def} that $\frac{1}{n}\sum_{b=1}^n \bar\beta^b_j \sim\mathcal{N}(\bar\beta_j, \sigma^2)$. Therefore, the improvement of this Bootstrapping process can be very limited.
% The only improvement of Bootstrapping in this case could come from the estimation of uncertainty. However, in the discussion of variable selection, the improvement of naive Bootstrapping TLSE is minor. 

We set the bound of the right hand side to be the same as TLSE estimate of $\hat K$. 
Recall the classical result of Bootstrap estimator from Wakefield \cite{wakefield2013bayesian} (c.f. Sec. 2.7.1).
\begin{lemma}
\label{lem:bootstrap_asymp}
A bootstrap estimator of the sample mean, $\mu$, of the distribution $F$ and assume $\E{F}<\infty$, and let the variance of $F$ be $\sigma^2$. Then we know that $\sqrt{n}(\bar Y_n-\mu) \xrightarrow[]{d}\mathcal{N}(0, \sigma^2)$, and for almost every sequence $Y_1, Y_2, ...$, 
\begin{align}
    \sqrt{n}(\bar Y^*_n - \bar Y_n) \xrightarrow[]{d}\mathcal{N}(0, \sigma^2). 
\end{align}
\end{lemma}

Applying Lemma \ref{lem:bootstrap_asymp}, and set $\bar\beta^*_j = \frac{1}{n}\sum_{b=1}^n \bar\beta_j^b$, we see that the naive bagging will enlarge the variance, resulting higher false discovery rate of $\hat K_{bag}$. The following remark summarizes the finding. 

\begin{remark}
The naive bagging OLS estimator $\bar\beta^*$ will enlarge the variance after integrating out $\bar\beta$ that 
\begin{align}
    var(\sqrt{n}(\bar\beta_j-\beta_j)) = \sigma^2(X_j^TX_j)^{-1},\;\;\;\; 
    var(\sqrt{n}(\bar\beta_j^*-\beta_j)) = 2\sigma^2(X_j^TX_j)^{-1}.
\end{align}
This will result in larger false discovery rates in $\hat K_{bag}$. 
\end{remark}

==> nonlinear_oscillator.tex <==
The damped cubic harmonic oscillator model can be characterized as following differential equations: 
\begin{align}
    \dot{u} = \alpha u^3 + \beta v^3 \\
    \dot{v} = \gamma v^3 + \delta u^3, 
\end{align}
where $\alpha=-0.1, \beta=-2.0, \gamma=2.0, \delta=-0.1$. We setup the initial condition as $[u_0, v_0]=[2,0]$. 
The number of measurement data are uniformly sampled from $t\in[0, 20]$ with increasing $n=[300, 400, 500,..., 800]$. 
We visualize the distributional evolution for the four active coefficient estimation in Fig.~\ref{fig:lotka}. For all four indices ($\Tilde{\alpha} u, \Tilde\beta uv, \Tilde\gamma v, \Tilde\delta uv$), we observe the distributional approximation would transit from an initially wrong distribution with biased mean and high variance to a delta function concentrating at the true value.

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{paper/figs/dist_converge_nonlinear.pdf}
    \caption{Empirical False discovery probability. }
    \label{fig:nonlinear}
\end{figure}

We further study the statistical properties of the Ensemble SINDy algorithm empirically. We replicate the E-SINDy algorithm for $50$ times with independently generated data. We illustrate the effect of BIP based uncertainty quantification for E-SINDy. 
As in Fig.~\ref{fig:nonlinear_stats}, when the noise level is low ($1\%$), the BIP inference consistently has the smallest bias with the smallest variance for the estimation. We note here the variance of the estimator scales with the level of noise in the environment. 
With an increasing level of noise, the bias and variance of the BIP estimator become progressively larger, resulting in increasing mean squared errors. 
It is easier for the estimated confidence interval to capture the ground truth under larger noise levels. 
This is because the bootstrap estimate may generate the confidence interval around a biased estimation. Therefore, the larger the noise level we have, the easier the truth value will be captured, by paying larger width in confidence interval estimate. 
Even if with a higher level of noise, it is inevitable that the MSE becomes worse. 
It is reassuring that the confidence interval would capture the ground truth, which is important for trustworthy inference and future predictions. 

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{paper/figs/phys_cubic_performance.pdf}
    \caption{Empirical False discovery probability. }
    \label{fig:nonlinear_stats}
\end{figure}

% Final polishing after getting subset estimation
